Quantum Hardware Roofline: Evaluating the Impact of Gate Expressivity on Quantum Processor Design

The design space of current quantum computers is expansive with no obvious winning solution. This leaves practitioners with a clear question: "What is the optimal system configuration to run an algorithm?". This paper explores hardware design trade-offs across NISQ systems to guide algorithm and hardware design choices. The evaluation is driven by algorithmic workloads and algorithm fidelity models which capture architectural features such as gate expressivity, fidelity, and crosstalk. We also argue that the criteria for gate design and selection should be extended from maximizing average fidelity to a more comprehensive approach that takes into account the gate expressivity with respect to algorithmic structures. We consider native entangling gates (CNOT, ECR, CZ, ZZ, XX, Sycamore, $\sqrt{\text{iSWAP}}$), proposed gates (B Gate, $\sqrt[4]{\text{CNOT}}$, $\sqrt[8]{\text{CNOT}}$), as well as parameterized gates (FSim, XY). Our methodology is driven by a custom synthesis driven circuit compilation workflow, which is able to produce minimal circuit representations for a given system configuration. By providing a method to evaluate the suitability of algorithms for hardware platforms, this work emphasizes the importance of hardware-software co-design for quantum computing.

==> sections/acknowledgements.tex <==
This work was supported by the DOE under contract DE-5AC02-05CH11231 through the Office of Advanced Scientific Computing Research (ASCR) Quantum Algorithms Team and
Accelerated Research in Quantum Computing programs, and by the NSF Challenge Institute for Quantum Computation(CIQC) program under award OMA-2016245.

==> sections/background.tex <==
\subsection{Quantum Computing Basics}
The fundamental unit of information in a quantum computer is the qubit, which can be represented as a vector of the form
\[
    | \psi \rangle = \alpha \begin{bmatrix} 1 \\ 0 \end{bmatrix} + \beta \begin{bmatrix} 0 \\ 1 \end{bmatrix}
\]
(ALSO ADD IN ABOUT DENSITY OPERATORS) where $\alpha$ and $\beta$ are complex numbers such that $|\alpha|^2 + |\beta|^2 = 1$ and $[ 1 \; 0 ]^T$ and $[ 0 \; 1 ]^T$ are orthonormal basis vectors representing two distinct quantum states.
The state of a quantum system with $n$ qubits in states $|\psi_1\rangle, |\psi_2\rangle, \dots |\psi_n\rangle$ lies in a $2^n \times 2^n$ Hilbert space, and can be represented by  the tensor product $|\psi_1\rangle \otimes |\psi_2\rangle \otimes \dots \otimes |\psi_n\rangle$.
This quantum state $|\psi\rangle$ can be evolved by use of $2^n \times 2^n$ unitary operators\cite{nielsen2002quantum}. \par
Universal quantum computing allows for any $2^n \times 2^n$ unitary operator to be applied. In practice, these arbitrary $n$-qubit unitaries are built of 1 qubit rotations and multi-qubit entangling gates. (Describe more about universal gates and different gate sets). 
\subsection{Fidelity}
Qubits are susceptible to various sources of error including gate errors, errors during initialization and measurement, and decoherence errors over time. All of these errors can collectively lead to a state that differs from the correct output state of an algorithm. The fidelity metric captures how closely the output state matches the calculated output state. In order to combat this loss in fidelity, quantum error correction allows one to encode a qubit into a set of qubits and correct for errors using several mid-circuit measurements. However, in the NISQ era of quantum computation, the state of the art ability to perform accurate mid circuit measurment and correction is too error prone to make QEC a viable tool. In this case, we must simply optimize for fidelity.

\subsubsection{Mathematical Definition of Fidelity}
Fidelity is defined by the following equation:

\[ \mathbf{F}(\rho, \sigma)  = \textbf{Tr}\sqrt{\sqrt{\rho}\sigma\sqrt{\rho}} \]

where $\rho$ represents the ideal quantum state and $\sigma$ represents the actual quantum state. This definition is symmetric, and a fidelity of 1 means that the states are identical. If we now consider a quantum circuit (add in things about quantum circuits and creating a quantum process). In order to measure fully measure quantum fidelity, we must use a technique known as process tomography. However, this method does not scale well and is susceptible to initialization and measurement errors. Because of this, metrics such as Randomized Benchmarking are used.

\subsubsection{Randomized Benchmarking}

In order to characterize a quantum machine, average fidelity of a quantum circuit is a more useful measure. Specifically, this is defined as the fidelity of a quantum process averaged over all inputs. The naive solution is to create randomly generate an input according to a Haar-random distribution, apply the quantum circuit, and then measure the fidelity of the output. However, there are several problems with this method. Randomly generating an input over the Haar measure is expensive, and measuring the fidelity of the output is generally intractable using tomography as mentioned before. In order to combat these issues, a technique known as Randomized Benchmarking was generated. \par

Randomized benchmarking consists of choosing random Clifford elements in such a way that they create an identity gate over n-qubits (this can be done efficiently due to the Gottesman-Knill theorem). Over a large set of these Clifford circuits, all of the error average to a basic depolarization channel. A Depolarization channel is on that goes from a state to a completely mixed state with probability $p$. This $p$ then becomes a measure of average \textbf{infidelity} in the circuit. If we vary the lengths of these random Clifford circuits, we can calculate the infidelity per gate ($p_{\text{gate}}$) . Taking 1 - $p_{\text{gate}}$ gives you the average fidelity, which can be thought of as the probability that a state does not succumb to any error when a gate is applied. We can see that maximizing the average fidelity 

\subsubsection{Cross Entropy Benchmarking}
In 2019, Google published a similar technique for computing average fidelity called cross entropy benchmarking (XEB). Once again, it takes advantage of the fact that the error over a set of random circuits becomes equivalent to a depolarization channel. (Research XEB theory in more detail later :(). This paper also shows that total average fidelity of a circuit can be approximated  very well by a simple digital error model. While this paper does not extend the validity of this model to very large circuits (since there are no machines of that size), we are still able to use that as the baseline model for our research.

==> sections/notes.tex <==
% \section{NOTES for writing}

% \begin{itemize}
% \item Methodology and metrics valid for FT - gate count still counts, fidelity may not be perfect..

% \item In some section we should contrast our ``expressivity'' metric (gate count) which is concrete and workload specific to the other metric which is ansatz specific and it is NOT quantitative (can't say anything if you compare two values).

%   \item \red{Figure with Weyl chamber and all gates we study. Some explanation, contrast Syc with CNOT.}
% \item 
 

% \end{itemize}

\section{Writing Notes}

\comment{\red{\subsection{Transpilation - this goes to end.}
Our benchmarking algorithms are all written in a standard gate set that includes CNOT gates and single qubit gates. In order to make claims across hardware, we must obtain the best representation of each algorithm for each gate set. In top-down synthesis techniques \cite{Qiskit, Cirq, sivarajah_tketrangle_2021}, there are standard rules to convert between different gate sets. For example, a CNOT can be broken down into a sequence of 2 Sycamore Gates and additional U3 gates. However, using such a rule to convert the entire algorithm ignores the patterns in the underlying unitary that can be exploited by different entangling gates. The BQSKIT transpilation tool, as outlined in \cite{younis_quantum_2022}, uses numerical instantiation on the unitary matrix encompassed by a block of qubits. By lifting the transpilation target from the given circuit to unitary, we eliminate the influence of the input circuit quality (see Figure \ref{fig:process}). While instantiation (as all numerical optimizers) are not guaranteed to be optimal, the results show that these state of the art techniques outperform direct rule transpilation across all gate sets and benchmarks \cite{younis_quantum_2022}.  We highlight these circuit structure patterns more in Section \ref{section:discussion}.}}


\red{\bf Costin: To say this in discussion or conclusion. Quantum is unlike classical. Classical benchmarking is influenced by domain level algorithmic optimizations, e.g. Linpack, HPGMG, HPCG. The result is not really influenced by compiler choice. In quantum, the result is determined by the compiler.}


\red{Find the paper that says synthesis increases gate parallelism. Say that our study may motivate new compiler optimizations: ->  we could come up with heuristics that increase para if motivated by the models.}

\red{\bf Make sure to add FT argument. Perf is T factories which address 1-q gates. 1-q count is determined by 2-q count. Hence all these considerations apply, models may need to be specialized.}


==> sections/trends.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Benchmark Suite} & \textbf{Benchmarks}           \\ \hline
QFT-based                & qft5, qft10                   \\ \hline
Hubbard                  & hubbard3x2                    \\ \hline
TFIM                     & tfim /tfxy16, tfim/tfxy 64    \\ \hline
QAE                      & qae 8, qae12, qae 15          \\ \hline
QPE                      & qpe 12, qpe 18, qpe 20        \\ \hline
VQE                      & vqe12 (LiH), vqe14 (LiBe3)    \\ \hline
Adder-based              & adder9, adder63, mul10, mul60 \\ \hline
Grover                   & grover5                       \\ \hline
QML                      & qml8, qml20                   \\ \hline
QAOA                     & qaoa5, qaoa10                 \\ \hline
\end{tabular}
\caption{Our suite of benchmarks used in the paper}
\label{tab:benchmarks}
\end{table}
